Zero-shot Sequential Neuro-symbolic Reasoning for Automatically Generating Architecture Schematic Designs

This paper introduces a novel automated system for generating architecture schematic designs aimed at streamlining complex decision-making at the multifamily real estate development project's outset. Leveraging the combined strengths of generative AI (neuro reasoning) and mathematical program solvers (symbolic reasoning), the method addresses both the reliance on expert insights and technical challenges in architectural schematic design. To address the large-scale and interconnected nature of design decisions needed for designing a whole building, we proposed a novel sequential neuro-symbolic reasoning approach, emulating traditional architecture design processes from initial concept to detailed layout. To remove the need to hand-craft a cost function to approximate the desired objectives, we propose a solution that uses neuro reasoning to generate constraints and cost functions that the symbolic solvers can use to solve. We also incorporate feedback loops for each design stage to ensure a tight integration between neuro and symbolic reasoning. Developed using GPT-4 without further training, our method's effectiveness is validated through comparative studies with real-world buildings. Our method can generate various building designs in accordance with the understanding of the neighborhood, showcasing its potential to transform the realm of architectural schematic design.

==> sec/Z_graveyard.tex <==

\subsection{Building Specification Generation}
A \emph{building specification} contains the number of floors, width and length of the building, a list of \emph{amenity specification}, and a list of \emph{unit specification}. An \emph{amenity specification} contains the type of the amenity, min and max area it could occupy, a list of preferred floors, and a list of alternative floors. A \emph{unit specification} contains the type of the unit (e.g., studio, one-bedroom, etc.), min and max percentage of total unit count, min and max area, and a list of length number of floors each containing the likelihood (from 0 to 5) of putting a unit on that floor. Here is an example of a \emph{building specification}:

\begin{verbatim}
{"n_floors": 12, "width": 25, "length": 64,
 "amenities": [{
   "type": "Entrance/Lobby", "min_area": 300, 
   "max_area": 500, "preferred_floors": [1],
   "alternative_floors": []}, ...]
 "units": [{
   "type": "Studio", "min_pct": 20, "max_pct": 30, 
   "min_area": 300, "max_area": 450, 
   "floors": [5, 5, 5, ..., 3, 3]}, ...]}
\end{verbatim}

Please see the supplemental material for the full prompts.

\subsection{Floor Assignment Generation}
Given the \emph{building specification}, the goal for the solver is to (1) determine the number of units for each type such that the ratio is within the specified range and (2) assign each unit and amenity to one of the floors while ensuring that we have enough space and have a wide area range for each floor, which gives the flexibility when solving for the layout. Here, we optimize for amenities being on the preferred floors and units being on floors with a high likelihood score. Here is an example of a \emph{floor assignment}:

\begin{itemize}
    \item Floor 1: Entrance/Lobby, Bicycle Storage, Package Room, 1 One-Bedroom, 6 Two-Bedroom
    \item Floor 2: Fitness Center, Laundry Room, Co-working Space, 4 One-Bedroom, 3 Two-Bedroom
    \item Floor 3: 15 Studio, 1 One-bedroom
    \item Floor 4: Rooftop Terrace, 1 One-Bedroom, 6 Two-Bedroom
\end{itemize}

We formulate this as a mixed integer linear programming (MILP) and use Gurobi to solve. Please see the supplemental material for details. If the solver could not find a solution, we ask the LLM to regenerate the building specification potentially widening the area and unit ratio ranges.

\subsection{LLM Feedback on Floor Assignment}
Since the solver does not know which lot it is optimizing for, we propose to add the feedback step where the LLM is tasked to evaluate the quality of the \emph{floor assignment}. Specifically, there is a trade-off between adding more amenities with a cost of having fewer units and vice versa. We then ask the LLM, using its expertise, to evaluate this trade-off and suggest modifications on the list of amenities. It can remove or modify existing amenities or propose a new amenity. We then run the floor assignment solver again and repeat until the LLM does not suggest any further modification. Please see the supplemental material for the full prompt.

\subsection{Adjacency Constraints Generation}
Once we have the final \emph{floor assignment}, we ask the LLM to give constraints between any two rooms on the same floor or constraints between a room and one of the four sides of the building. Here is the example list of adjacency constraints:
\begin{verbatim}
{1: [["Entrance/Lobby", "SouthWall"], 
     ["Entrance/Lobby", "Bicycle Storage"]],
 2: [["Fitness Center", "Laundry Room"],
     ["One-Bedroom A", "One-Bedroom B"]], ...}
\end{verbatim}

\subsection{Floor Plan Generation}
In this stage, given the \emph{floor assignment} and the adjacency constraints, we aim to construct a floor plan for each floor. To simplify, we model every amenity and unit as an axis aligned rectangle where the design variables are the position and the dimension of the rectangle. In addition, we allocate an elevator/stair space that spans vertically across all floors. The position of the elevator/stair is another design variable. In addition to the given adjacency constraints, we constrain that no two rooms intersect, the ratio between width and height is less than 2.7, and a unit has to be adjacent to one of the walls to accommodate at least one window. We maximize the space utilization. We formulate this problem as a mixed integer quadratic programming (MIQP) problem and solve using Gurobi. Please see the supplemental material for details.

\subsection{Solver Feedback on Adjacency Constraint}
Since the LLM lacks spatial understanding, it may output adjacency constraints that are impossible for the solver to generate a valid solution -- that is, the constraints are unsatisfiable (also known as ``unsat''). While this can be used as feedback for the LLM to regenerate the constraints, such feedback is best if it includes specific reasons for failure. To solve this, we ask Gurobi to output an irreducible inconsistent subsystem (IIS), which is the smallest subset of constraints that make the problem infeasible. If the IIS contains conflicting adjacency constraints, we can precisely ask the LLM to remove one of the conflicting constraints.

\subsection{LLM Prompting and Validation}
For each request we ask the LLM, we specifically ask it to output a JSON string which can easily be parsed. To ask it to output a specific schema, we provide an example JSON with the format we wanted with generic values. For example, to get the \emph{amenity specification}, we append the following at the end:
\begin{verbatim}
Output in the following JSON format:
```json
[{"type": "a", "min_area": 1, "max_area": 1,
"preferred_floors": [1], "alternative_floors": [2, 3]}]
```
\end{verbatim}
When parsing responses, we perform thorough checks for the data types and value ranges for each field and provide precise feedback on any parsing error. We repeat the correction process for up to five times before we give up.
